Enhance Hyperbolic Representation Learning via Second-order Pooling

Hyperbolic representation learning is well known for its ability to capture hierarchical information. However, the distance between samples from different levels of hierarchical classes can be required large. We reveal that the hyperbolic discriminant objective forces the backbone to capture this hierarchical information, which may inevitably increase the Lipschitz constant of the backbone. This can hinder the full utilization of the backbone's generalization ability. To address this issue, we introduce second-order pooling into hyperbolic representation learning, as it naturally increases the distance between samples without compromising the generalization ability of the input features. In this way, the Lipschitz constant of the backbone does not necessarily need to be large. However, current off-the-shelf low-dimensional bilinear pooling methods cannot be directly employed in hyperbolic representation learning because they inevitably reduce the distance expansion capability. To solve this problem, we propose a kernel approximation regularization, which enables the low-dimensional bilinear features to approximate the kernel function well in low-dimensional space. Finally, we conduct extensive experiments on graph-structured datasets to demonstrate the effectiveness of the proposed method.

==> tables/table1.tex <==
\begin{tabular}{clccccccccccccccc} 
\arrayrulecolor{black}\toprule
&\multicolumn{1}{c}{\multirow{2}{*}{\textsc{Method}}} & \multicolumn{3}{c}{\textsc{ACC}}   & \multicolumn{3}{c}{\textsc{AUC-ROC}} & \multicolumn{3}{c}{\textsc{NMI}} &  \multicolumn{3}{c}{\textsc{ARI}} & \\ 
\cmidrule(lr){3-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}\cmidrule(lr){12-14}
&& \textsc{Cora}   & \textsc{CiteSeer} & \textsc{PubMed} 
& \textsc{Cora}   & \textsc{CiteSeer} & \textsc{PubMed}
& \textsc{Cora}   & \textsc{CiteSeer} & \textsc{PubMed}
& \textsc{Cora}   & \textsc{CiteSeer} & \textsc{PubMed}  \\

\arrayrulecolor{black}\midrule
\parbox[t]{3mm}{\multirow{9}{*}{\rotatebox[origin=c]{90}{\textsc{Public Split}}}} 
&GCN & 81.46±0.63 & 71.28±0.65 & 79.30±0.34 & 96.67±0.09 & 89.99±0.09 & 91.66±0.21 & 60.32±1.21 & 44.51±0.67 & 39.35±0.59 & 62.66±1.09 & 46.44±0.99 & 45.94±0.71 \\
&GAT & 80.20±0.54 & 70.97±0.85 & 78.27±0.54 & 96.33±0.27 & 90.46±0.08 & 91.68±0.17 & 58.13±1.07 & 44.32±0.70 & 37.31±1.20	& 59.40±0.79 & 46.78±0.64 & 43.85±1.07\\
&SAGE & 81.20±0.50 & 71.24±0.38 & 77.18±0.69 & 96.44±0.05 & 
 89.53±0.03 & 90.82±0.30 & 59.92±0.77 & 43.87±0.52 & 35.70±1.30 & 61.53±1.13 & 46.37±0.64 & 41.68±1.54\\
&Transformer& 80.06±0.47 & 70.68±0.40 & 76.62±0.53 & 96.19±0.05 & 89.78±0.13 & 90.75±0.19 & 57.81±0.68 & 43.36±0.65 & 34.63±0.94 & 59.48±0.70 &	45.61±0.77	& 40.37±1.07\\
&GCNII & 84.78±0.27 & 71.64±0.38 & 79.54±0.39 & 97.50±0.22 & 90.46±0.61 & 92.26±0.26 & 66.34±0.21 & 45.73±0.58 & 39.86±0.57 & 69.94±0.48 & 47.58±0.74 & 46.56±0.90 \\

\arrayrulecolor{black!30}\cmidrule{2-14}
&HGCN(*)  & 78.82±1.07 & - & 75.38±0.25 & 95.44±0.49 & - & 89.96±0.20 & 56.67±1.80 & - & 32.99±0.46 & 57.79±2.56 & - & 38.38±0.41 \\
&HGCN(Ours)  & 79.63±0.42 & 69.07±0.79  & 77.87±0.82 & 95.36±0.09 & 87.87±0.47 & 90.47±0.44 & 57.61±0.33 & 42.77±0.67 &37.53±1.50& 58.51±1.02 & 44.90±0.55 &  43.59±1.77\\
&HGCNII (Ours)  & 84.63±0.29 & 72.87±0.76 & 79.97±0.53  &97.30±0.13 & 90.33±0.28& 92.11±0.09& 65.95±0.65 &47.01±0.33 & 41.55±0.87 & 68.61±0.35 & 49.34±1.19 & 47.83±1.11\\

\arrayrulecolor{black!30}\cmidrule{2-14}

&HBP-GCNII  & 83.94±0.49 & 71.01±0.90 & 78.32±0.42 & 97.27±0.09 & 90.34±0.24 & 91.99±0.19 & 65.18+0.32 & 46.43±0.40 & 40.92±0.70 & 67.26+0.90 & 48.97±1.17 & 47.47±0.84 \\
&HBCP-GCNII  & 84.63±0.91 &72.77±0.39 & 79.50±0.36\\


&HLBP-GCNII & 84.38±0.82 & 73.74±0.42 & 80.24±0.49 & 97.50±0.07 & 90.91±0.11 & 92.61±0.08 & 65.49±1.54 & 47.33±0.54 & 41.80±0.75 & 68.28±1.40 & 50.51±0.91 & 48.22±0.92\\
&HBPU-GCNII  & 84.26±0.38 & 72.94±0.65 & 79.98±0.30 & 97.28±0.08 & 90.34±0.14 & 91.96±0.11 & 65.25±0.72 & 46.13±0.58 & 40.83±0.76 & 67.44±0.68 & 49.01±0.91 & 47.61±0.82\\
&HA-GCNII  &  85.30±0.16 & 73.80±0.62 & 79.70±0.78 \\
&HBPA-GCNII  &  83.77±0.45 & 72.27±0.05 & 79.83±0.34\\
&HAU-GCNII  & 85.40±0.29 & 73.50±0.36 & 79.70±0.71 \\
&HBPAU-GCNII  &  84.17±0.31 & 72.57±0.77 & 80.17±0.09 \\

\arrayrulecolor{black!30}\cmidrule{2-14}
& BP-GCNII &  83.80±0.30 & 70.97±0.56   & 78.50±0.16    &  97.11±0.08  &  89.44±0.21 &  91.42±0.18 &  64.32±0.88 & 44.35±0.30 & 38.33±0.25  & 67.60±0.50 & 46.08±0.81 & 43.83±0.50\\ 
& BCP-GCNII &  84.72±0.58 & 71.57±0.80 & NaN\\ 
& BP-GAT &  80.13±1.18 &  69.17±0.93 & 78.10±0.78 \\ 
& CP-GAT &  75.90±0.72 & 69.40±1.85 & 79.07±0.78 \\ 
& BCP-GAT & 80.07±1.55 &  69.67±0.45 & 78.57±0.29 \\ 
& BP-Transf & 74.47±3.61 & 55.50±4.13 & 72.27±0.32  \\ 
& CP-Transf &  78.97±0.90 & 70.23±1.69 & 77.30±0.52 \\ 
& BCP-Transf & 77.47±2.58 & 61.70±4.16 & 70.37±1.87  \\ 
& HBP-Transf &  81.03±0.12 & 65.50±1.21 & 77.43±0.45 \\ 
& HBCP-Transf &  80.57±0.09 & 66.13±3.42 & 77.57±0.57\\ 
\arrayrulecolor{black}\bottomrule
\end{tabular}


==> tables/table11.tex <==
\begin{tabular}{lcccc} 
\arrayrulecolor{black}\toprule
{\textsc{Method}} 

 & \textsc{PubMed} &\textsc{Citeseer}   & \textsc{Cora}  \\

\arrayrulecolor{black}\midrule

 HBP-GCNII (64dim) & 80.3$\pm$0.6 & 73.3$\pm$0.3& 84.8$\pm$0.4 \\
\arrayrulecolor{black!30}\cmidrule{1-4}
 HBP-GCNII$_\text{LOW-RANK}$ (16dim) & 80.2$\pm$0.5 & 73.7$\pm$0.4 & 84.3$\pm$0.8 \\

\arrayrulecolor{black}\bottomrule
\end{tabular}


==> tables/table3.tex <==
\begin{tabular}{clccccccccccccccc} 
\arrayrulecolor{black}\toprule
&\multicolumn{1}{c}{\multirow{2}{*}{\textsc{Method}}} & \multicolumn{3}{c}{\textsc{ACC}}   & \multicolumn{3}{c}{\textsc{AUC-ROC}} & \multicolumn{3}{c}{\textsc{NMI}} &  \multicolumn{3}{c}{\textsc{ARI}} & \\ 
\cmidrule(lr){3-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}\cmidrule(lr){12-14}
&&\textsc{Cora}   & \textsc{CiteSeer} & \textsc{PubMed} 
& \textsc{Cora}   & \textsc{CiteSeer} & \textsc{PubMed}
& \textsc{Cora}   & \textsc{CiteSeer} & \textsc{PubMed}
& \textsc{Cora}   & \textsc{CiteSeer} & \textsc{PubMed}  \\

\arrayrulecolor{black}\midrule

\parbox[t]{3mm}{\multirow{9}{*}{\rotatebox[origin=c]{90}{\textsc{Full Split}}}} 
&GCN & 87.14±0.54 & 78.82±1.04 & 87.94±0.50 & 97.90±0.31 & 93.34±0.06 & 96.40±0.18 & 70.01±0.72 & 55.34±0.97 & 57.57±1.08 & 73.62±1.30 & 58.42±1.20 & 67.02±1.21  \\
&GAT & 83.06±0.60 & 76.56±0.34 & 84.40±0.28 & 97.03±0.03 & 92.87±0.16 & 95.75±0.03 & 62.72±1.00 & 52.92±0.70 & 49.55±0.60 & 66.00±1.16 & 55.80±0.60 & 58.44±0.72\\
&SAGE & 87.68±0.35 & 79.22±0.52 & 88.08±0.27 & 97.89±0.05 & 93.07±0.09 & 97.22±0.23 & 70.85±0.59 & 55.01±0.86 & 57.92±0.68	& 74.65±0.84 & 	58.26±0.94 & 66.82±0.59\\
&Transformer & 87.00±0.37 & 79.54±0.35 & 88.78±0.40 & 97.87±0.01 & 93.30±0.14 & 97.41±0.17 & 69.99±0.69 & 55.73±0.58 & 59.78±1.04 & 73.52±0.71 & 58.72±0.63 & 68.62±0.97\\
&GCNII & 82.10±3.10 & 77.12±0.22 & 85.62±0.55 & 96.92±0.37 & 92.64±0.38 & 95.57±0.10 & 66.39±3.08 & 53.99±0.34 & 52.90±1.12 & 66.98±2.81 & 56.69±0.45 & 61.54±1.28 \\ 

\arrayrulecolor{black!30}\cmidrule{2-14}
&HGCN (Ours) &	79.87±3.41  &  75.27±0.50 & 88.17±0.41 &  96.26±0.73 & 90.43±0.22 & 96.74±0.04 & 65.02±1.36 & 51.38±0.19 & 60.18±0.94 & 68.08±2.10 & 53.67±0.04 & 69.44±0.92\\
&HGCNII (Ours) & 82.00±0.79	& 76.73±0.17 & 85.20±0.22 & 97.05±0.10 & 90.84±0.17 & 95.75±0.02 & 66.39±0.35  & 53.61±0.19   & 51.95±0.69  &  66.63±0.85  &  56.04±0.25 &  60.55±0.54 \\

\arrayrulecolor{black!30}\cmidrule{2-14}

&HBP-GCNII & 87.76±0.36 & 77.44±0.11 & 85.54±0.17 & 98.10±0.05 & 91.49±0.22 & 95.88±0.03 & 71.90±0.43 & 54.64±0.22 & 52.62±0.41 & 74.93±0.73 & 57.37±0.22 & 61.44±0.43\\
&HBCP-GCNII & 88.57±0.05 & 77.10±0.08 &  85.80±0.08 \\

&HLBP-GCNII & 85.64±0.61 & 76.92±0.30 & 84.90±0.14 & 97.79±0.08 & 91.92±0.23 & 95.82±0.02 & 69.77±0.72 & 57.52±0.86 & 51.19±0.29 & 71.59±1.26 & 58.27±0.73 & 60.03±0.39\\
&HBPU-GCNII & 88.56±0.42 & 78.48±0.38 & 87.46±0.11 & 98.19±0.14 & 93.01±0.10 & 96.31±0.06 & 72.74±0.68 & 55.28±0.50 & 56.53±0.33 & 77.03±0.88 & 58.62±0.49 & 66.17±0.29\\
&HA-GCNII  &  77.57±0.29 & 77.07±0.29 & 84.60±0.08\\
&HBPA-GCNII & 89.43±0.26 & 78.50±0.14 & 87.93±0.29 & \\
&HAU-GCNII  & 78.60±1.00 & 77.03±0.17 & 84.50±0.08\\
&HBPAU-GCNII & 89.37±0.46  & 78.60±0.16 & 87.20±0.29  & \\

\arrayrulecolor{black!30}\cmidrule{2-14}
& BP-GCNII &  87.77±0.91 & 59.53±2.58 & 87.63±0.05  &  97.61±0.24 & 85.22±2.35  & 95.89±0.04  &  71.80±1.26 & 41.59±2.31 & 56.83±0.25 &  75.59±1.40 & 36.88±3.65 & 66.55±0.14\\ 
& BCP-GCNII &  88.04±0.21 & 77.63±0.29 & NaN \\ 
& BP-GAT & 86.10±0.35 & 77.97±0.23 & 86.70±0.35\\ 
& CP-GAT &  82.30±0.82 & 76.10±0.82 & 84.10±0.36\\ 
& BCP-GAT & 85.47±0.40 & 76.90±0.35 & 86.00±0.26\\ 
& BP-Transf &  83.83±1.47 & 74.43±1.62 & 89.53±0.42\\ 
& CP-Transf & 84.60±0.44 & 78.43±0.15 & 88.77±0.21 \\ 
& BCP-Transf & 84.87±0.45 & 75.77±0.91 & 89.63±0.06\\ 
& HBP-Transf & 86.07±0.29 & 76.70±0.43 & 89.13±0.29 \\ 
& HBCP-Transf & 86.33±0.21 &  76.10±0.36 &  88.90±0.22 \\ 

\arrayrulecolor{black}\bottomrule \\

\parbox[t]{3mm}{\multirow{9}{*}{\rotatebox[origin=c]{90}{\textsc{Complete Split}}}} 
&GCN & 88.76±1.01 & 78.36±0.30 & 87.76±0.65 & 97.87±0.37 & 94.19±0.11 & 96.86±0.19 & 73.24±1.32 & 58.60±0.58 & 57.72±1.49 & 76.25±2.23 & 60.17±0.46 & 66.14±1.61 \\
&GAT & 83.16±1.04 & 76.80±0.63 & 82.60±0.37 & 96.84±0.10 & 93.52±0.18 & 95.72±0.03 & 64.13±1.50 & 57.33±1.06 &	46.38±0.94 & 64.69±3.00 & 58.20±1.07 & 54.05±0.92 \\
&SAGE & 89.64±0.43 & 78.48±0.18 & 87.44±0.38 & 97.86±0.06 & 93.49±0.04 & 97.56±0.28 & 74.63±0.83 & 57.72±0.40 & 56.80±0.91 & 77.11±1.10 & 59.15±0.16 & 65.25±1.03\\
&Transformer & 89.88±0.30 & 79.36±0.17 & 88.00±0.40 & 98.02±0.07 & 93.64±0.11 & 97.80±0.26 & 75.25±0.84 & 58.96±0.34 & 58.41±1.01 & 77.62±0.65 & 60.71±0.36 & 66.72±0.98\\
&GCNII & 84.16±2.27 & 76.76±0.65 & 85.44±0.70 & 96.82±0.42 & 92.86±0.39 & 96.13±0.07 & 68.33±1.91 & 57.92±1.08 &	52.86±1.42 & 70.83±1.16 & 58.14±1.26 & 60.61±1.79 \\ 

\arrayrulecolor{black!30}\cmidrule{2-14}
&HGCN (Ours) &	 84.80±3.12 & 76.67±0.62 & 88.07±0.09 & 97.23±0.51 & 90.54±0.31 & 97.52±0.04 & 72.93±0.91 & 56.79±0.54 & 58.78±0.68 &  75.70±0.84 & 58.26±0.71 & 67.49±0.71\\
&HGCNII (Ours) &	84.27±0.68 & 76.93±0.25 & 84.73±0.25 & 96.63±0.11 &  90.44±0.37 & 96.10±0.02 & 68.65±0.91 & 57.75±0.40  & 51.63±0.86 & 70.81±0.52 & 58.39±0.46 & 59.17±0.56\\
&HA-GCNII  &  81.27±0.62 & 77.13±0.09 & 83.80±0.28 \\
&HBPA-GCNII  & 90.67±0.41 &  78.73±0.09   & 87.60±0.57 \\
&HAU-GCNII  & 81.13±0.52 & 76.80±0.57 & 83.87±0.19\\
&HBPAU-GCNII  & 90.33±0.50 & 78.13±0.25  & 88.13±0.25\\
\arrayrulecolor{black!30}\cmidrule{2-14}

&HBP-GCNII & 88.96±0.43 & 77.16±0.54 & 85.04±0.38 & 97.69±0.08 & 91.43±0.17 & 96.34±0.03 & 74.50±1.04 & 57.92±1.27 & 52.52±0.82 & 77.46±0.65 & 58.84±1.04 & 59.85±0.90\\
&HBCP-GCNII &  89.40±0.16 & 77.73±0.25 & 85.27±0.25 \\
&HLBP-GCNII & 86.76±0.65 & 76.92±0.30 & 84.24±0.33 & 97.58±0.04 & 91.92±0.23 & 96.13±0.05 & 71.25±0.85 & 57.52±0.86 & 50.66±0.82 & 73.42±1.10 & 58.27±0.73 & 58.05±0.77\\
&HBPU-GCNII & 89.76±0.36 & 78.20±0.24 & 87.24±0.38 & 98.06±0.33 & 92.99±0.42 & 96.81±0.04 & 75.27±0.72 & 59.34±0.88 & 57.16±0.85 & 79.20±0.46 & 60.37±0.57 & 65.59±0.91\\

\arrayrulecolor{black!30}\cmidrule{2-14}
& BP-GCNII & 88.33±0.90 & 58.60±9.20 & 88.27±0.41 & 97.97±0.11 & 85.83±3.07 & 96.82±0.01 &  73.56±1.57 & 42.95±5.36  & 58.60±0.91  &  76.30±0.80 & 35.04±9.60 & 67.90±1.08\\ 
& BCP-GCNII & 89.53±0.12 & 77.07±0.61 & 86.20±0.53\\ 
& BP-GAT & 88.40±0.53 & 77.87±0.61 & 85.67±0.50 \\ 
& CP-GAT &  83.27±1.22 & 76.13±0.83 & 83.47±0.81\\ 
& BCP-GAT & 86.07±0.42 & 77.40±0.20 & 84.87±0.50\\ 
& BP-Transf &  87.33±0.99 & 74.47±3.37 & 90.20±1.25\\ 
& CP-Transf & 85.00±0.40  & 78.87±0.41 & 88.33±0.12\\ 
& BCP-Transf & 87.67±0.61 &  77.00±1.25 & 90.67±0.46\\ 
& HBP-Transf & 89.33±0.25 & 78.13±0.41 & 88.67±0.47\\
& HBCP-Transf &  89.13±0.41 & 77.93±0.62 & 88.87±0.52\\ 
\arrayrulecolor{black}\bottomrule
\end{tabular}


==> tables/table4.tex <==
\begin{tabular}{clccc} 
\arrayrulecolor{black}\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\textsc{}}} & \multicolumn{1}{c}{\multirow{2}{*}{\textsc{Method}}} &\multicolumn{3}{c}{\textsc{Accuracy (\%)}}  \\ 
\cmidrule(lr){3-5}
& &\textsc{Cora}   & \textsc{CiteSeer} & \textsc{PubMed} \\

\arrayrulecolor{black}\midrule
\multirow{3}{*}{{\textsc{$\delta=10^{-2}$}}} & HBP-GNN  & 83.18±0.54 & 71.30±0.94 & 79.54±0.55 \\
&HLBP-GNN & 84.46±0.40 & 71.96±0.74 & 79.84±0.33\\
&HBPU-GNN  & 83.28±0.59 & 71.20±0.99 & 77.46±1.62\\
% \arrayrulecolor{black!30}\cmidrule{1-5}
% \multirow{3}{*}{{\textsc{$\delta=10^{-1}$}}} & HBP-GNN  & 83.60±0.46 & 72.10±0.78 & 80.00±0.46   \\
% &HLBP-GNN &  84.42±0.34 & 72.84±0.51 & 80.04±0.22\\
% &HBPU-GNN  &  83.82±0.39 & 71.90±0.60 & 79.64±0.39  \\
\arrayrulecolor{black!30}\cmidrule{1-5}
\multirow{3}{*}{{\textsc{$\delta=1$}}} &HBP-GNN  &  83.64±0.74 & 72.48±0.77 & 80.02±0.30 \\
&HLBP-GNN &  84.44±0.61 & 73.48±0.58 & 80.28±0.53\\
&HBPU-GNN  & 83.98±0.45 & 72.64±0.36 & 79.98±0.54 \\
% \arrayrulecolor{black!30}\cmidrule{1-5}
% \multirow{3}{*}{{\textsc{$\delta=10$}}} &HBP-GNN  & 83.76±0.46 & 72.58±0.82 & 79.98±0.51  \\
% &HLBP-GNN &  84.18±0.51 & 73.30±0.60 & 80.38±0.29\\
% &HBPU-GNN  & 83.92±0.41 &  73.46±0.61 & 80.40±0.71 \\
\arrayrulecolor{black!30}\cmidrule{1-5}
\multirow{3}{*}{{\textsc{$\delta=10^{2}$}}} & HBP-GNN  &  82.54±0.71 & 66.52±5.73 & 80.18±0.33\\
&HLBP-GNN &  82.02±2.93 & 73.72±0.56 & 80.14±0.42\\
&HBPU-GNN  &  82.56±1.29 & 51.84±16.00 & 79.62±0.99\\
\arrayrulecolor{black}\bottomrule
\end{tabular}




==> tables/table5.tex <==
\begin{tabular}{llccc} 
\arrayrulecolor{black}\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\textsc{Core}}}
 &\multicolumn{1}{c}{\multirow{2}{*}{\textsc{Method}}} &\multicolumn{3}{c}{\textsc{Accuracy (\%)}}  \\ 
\cmidrule(lr){3-5}
& &\textsc{Cora}   & \textsc{CiteSeer} & \textsc{PubMed} \\

\arrayrulecolor{black}\midrule
\multirow{3}{*}{{\textsc{GCN}}}
&Euclidean-GCN  &  81.46±0.63 & 71.28±0.65 & 79.30±0.34 \\
&HBP-GCN  & 78.12±1.12 &  62.98±2.90 & 52.14±0.25 \\
&HLBP-GCN &  &  &\\
&HBPU-GCN  &  &  &\\
\arrayrulecolor{black!30}\cmidrule{1-5}
\multirow{3}{*}{{\textsc{GCNII}}}
&Euclidean-GCNII  & 83.94±0.49 & 71.01±0.90 & 78.32±0.42  \\
&HBP-GCNII & 83.94±0.49 & 71.01±0.90 & 78.32±0.42  \\
&HLBP-GCNII & 84.38±0.82 & 73.74±0.42 & 80.24±0.49\\
&HBPU-GCNII  &  84.26±0.38 & 72.94±0.65 & 79.98±0.30 \\
\arrayrulecolor{black!30}\cmidrule{1-5}
\multirow{3}{*}{{\textsc{SAGE}}}
&Euclidean-SAGE  &   81.20±0.50 & 71.24±0.38 & 77.18±0.69\\
&HBP-SAGE  &  77.78±0.90  & 64.96±1.69 & 76.52±0.41\\
&HLBP-SAGE &   &  & \\
&HBPU-SAGE  &   &  & \\

\arrayrulecolor{black}\bottomrule
\end{tabular}


==> tables/table7.tex <==
    \begin{tabular}{lcccccccc}
        \toprule
        \begin{tabular}{c}\textbf{Dataset} \\\textbf{hyperbolicity}($\delta$)\end{tabular} & \multicolumn{2}{c}{\begin{tabular}{c}\textbf{Airport} \\($\delta = 1$)\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}{c}\textbf{PubMed} \\($\delta = 3.5$)\end{tabular}}  & \multicolumn{2}{c}{\begin{tabular}{c}\textbf{CiteSeer} \\($\delta = 5$)\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}{c}\textbf{Cora} \\($\delta =11$)\end{tabular}}\\
        \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
        \textbf{Task} & \textbf{LP} & \textbf{NC} & \textbf{LP} & \textbf{NC} & \textbf{LP} & \textbf{NC} & \textbf{LP} & \textbf{NC} \\
        \midrule
        % MLP & 89.81$\pm$0.56 & 68.90$\pm$0.46 & 83.33$\pm$0.56 & 72.40$\pm$0.21 & 93.73$\pm$0.63 & 59.53$\pm$0.90 & 83.33$\pm$0.56 & 51.59$\pm$1.28 \\
        % HNN & 90.81$\pm$0.23 & 80.59$\pm$0.46 & 94.69$\pm$0.06 & 69.88$\pm$0.43 & 93.30$\pm$0.52 & 59.50$\pm$1.28 & 90.92$\pm$0.40 & 54.76$\pm$0.61 \\
        % \arrayrulecolor{black!30}\cmidrule{1-9}
        
        GCN             & 97.1$\pm$0.4 & 81.5$\pm$0.6 & 89.5$\pm$3.6 & 79.3$\pm$0.3 & 82.5$\pm$1.9 &  71.3$\pm$0.7 & 90.4$\pm$0.2 & 81.4$\pm$0.6 \\
        GCNII           & 96.2$\pm$0.5 & 83.7$\pm$0.9  & 96.5$\pm$0.3  &  79.5$\pm$0.4 & 92.3$\pm$0.5  & 71.6$\pm$0.4 & 96.1$\pm$0.5 &  84.4$\pm$0.3\\
        GAT             & 95.8$\pm$0.2 & 82.7$\pm$0.4 & 91.4$\pm$1.8 & 78.2$\pm$0.5 & 86.5$\pm$1.5 & 70.9$\pm$0.8 & 93.2$\pm$0.2 & 80.2$\pm$0.5 \\
        GraphSAGE       & 93.4$\pm$0.5 & 82.2$\pm$0.4 & 86.2$\pm$0.8 & 77.2$\pm$0.7 & 92.0$\pm$0.4 & 71.2$\pm$0.4 & 85.5$\pm$0.5 & 81.2$\pm$0.5 \\
        TransformerConv & 96.4$\pm$0.4 &  83.3$\pm$0.1 & 84.6$\pm$1.1  & 76.6$\pm$0.5  & 78.2$\pm$1.4  & 70.7$\pm$0.4  & 87.9$\pm$0.9 &  80.1$\pm$0.5\\
        \arrayrulecolor{black!30}\cmidrule{1-9}
        
        HGCN~\cite{chami2019hyperbolic} & 96.4$\pm$0.1 & 90.6$\pm$0.2 & 96.3$\pm$0.1 & 80.3$\pm$0.3 & 96.6$\pm$0.0 & 68.0$\pm$0.6 & 92.9$\pm$0.1 & 79.9$\pm$0.2 \\
        HAT~\cite{zhu2020graph} & 97.9$\pm$0.1 & 89.6$\pm$1.0 & 94.2$\pm$0.2 & 77.4$\pm$0.7 & 95.8$\pm$0.4 & 68.6$\pm$0.3 & 94.0$\pm$0.2 & 78.3$\pm$1.4 \\
        GIL~\cite{zhu2020graph} & {98.8$\pm$0.3 }& 91.3$\pm$0.8 & 95.5$\pm$0.2 & 78.9$\pm$0.3 & \textbf{99.8$\pm$0.4 }& 73.0$\pm$0.7 & {98.3$\pm$0.8} & 83.6$\pm$0.6 \\
        H2H-GCN~\cite{dai2021hyperbolic} & 96.7$\pm$0.1 & 91.0$\pm$0.3&97.1$\pm$0.1 & {82.3$\pm$0.4} & - & - &95.4$\pm$0.1& 83.6$\pm$0.8\\
        % ACE-HGNN~\cite{fu2021ace} &-&-& 95.0$\pm$0.0 & 84.2$\pm$0.0&96.9$\pm$0.0 & 85.3$\pm$0.0 & 93.5$\pm$0.0& 83.9$\pm$0.0\\
        {DeepHGCN}~\cite{liu2023deephgcn} & {98.1$\pm$0.3} & {94.7$\pm$0.9} & {96.1$\pm$0.2} & {79.4$\pm$0.9} & {97.4$\pm$0.4} & {73.3$\pm$0.7} & {93.9$\pm$0.8} & {83.6$\pm$0.4} \\
        \arrayrulecolor{black!30}\cmidrule{1-9}
        
        HBP ($64^2$dim.) & 97.4$\pm$0.4& 91.8$\pm$0.1& {97.7$\pm$0.2} & 80.3$\pm$0.6 & 99.1$\pm$0.3 & {73.3$\pm$0.3} & {\textbf{98.4$\pm$0.4}} & {84.8$\pm$0.4}\\
        HBP-$\mathbb{KR}$ ($256$dim.) & \textbf{98.9$\pm$0.1} & \textbf{94.9$\pm$0.2} & \textbf{97.8$\pm$0.2} & \textbf{82.7$\pm$0.6} & {99.2$\pm$0.3} & \textbf{74.4$\pm$0.4} & 98.3$\pm$0.1  &   \textbf{85.6$\pm$0.3} \\
        \arrayrulecolor{black}\bottomrule
    \end{tabular}
